Text mining and sentiment analysis of COVID-19 tweets

The human severe acute respiratory syndrome coronavirus 2 (SARS-Cov-2), causing the COVID-19 disease, has continued to spread all over the world. It menacingly affects not only public health and global economics but also mental health and mood. While the impact of the COVID-19 pandemic has been widely studied, relatively fewer discussions about the sentimental reaction of the population have been available. In this article, we scrape COVID-19 related tweets on the microblogging platform, Twitter, and examine the tweets from Feb~24, 2020 to Oct~14, 2020 in four Canadian cities (Toronto, Montreal, Vancouver, and Calgary) and four U.S. cities (New York, Los Angeles, Chicago, and Seattle). Applying the Vader and NRC approaches, we evaluate the sentiment intensity scores and visualize the information over different periods of the pandemic. Sentiment scores for the tweets concerning three anti-epidemic measures, masks, vaccine, and lockdown, are computed for comparisons. The results of four Canadian cities are compared with four cities in the United States. We study the causal relationships between the infected cases, the tweet activities, and the sentiment scores of COVID-19 related tweets, by integrating the echo state network method with convergent cross-mapping. Our analysis shows that public sentiments regarding COVID-19 vary in different time periods and locations. In general, people have a positive mood about COVID-19 and masks, but negative in the topics of vaccine and lockdown. The causal inference shows that the sentiment influences people's activities on Twitter, which is also correlated to the daily number of infections.

==> tables/DeathDefinition.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\caption{The results of the augmented Dickey-Fuller test \label{tab:deathdef}}
\begin{tabular}{lccccclccccc}
\hline
             & \multicolumn{2}{c}{British Columbia}                                    &  & \multicolumn{2}{c}{Ontario} &  & \multicolumn{2}{c}{Quebec}                                     &                      & \multicolumn{2}{c}{Alberta}                                    \\ \cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
Definition   & Differencing                           & lag $p$                        &  & Differencing     & lag $p$  &  & \multicolumn{1}{l}{Differencing} & \multicolumn{1}{l}{lag $p$} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{Differencing} & \multicolumn{1}{l}{lag $p$} \\ \hline
Definition 1 & 1 degree & 1 &  & 1 degree         & 1        &  & 1 degree                         & 1                           &                      & 1 degree                         & 1                           \\
             & no differencing                        & 2                              &  & -                & -        &  & - & -                           &                      & -                                & -                           \\ 
Definition 2 & 1 degree                               & 2                              &  & no differencing  & 2        &  & 1 degree                         & 2                           &                      & 1 degree                         & 1                           \\
Definition 3 & 1 degree                               & 1                              &  & 1 degree         & 4        &  & -                                & -                           &                      & -                                & -                           \\
\hline
\end{tabular}
\end{table}

==> tables/Tab_Peh_AR.tex <==
\begin{sidewaystable}
\setlength\extrarowheight{1pt} % provide a bit more vertical whitespace
\centering
\captionsetup{size=small}
\tiny

\begin{threeparttable}
\caption[]{The observed prediction error and expected prediction error for different lag order of autoregressive models.}
\label{Tab:Table-Peh-AR}

\begin{tabular}{lllccccccccccccc}
\hline
                                &                                &                                            & \multicolumn{6}{c}{Observed Prediction Error}                      &  & \multicolumn{6}{c}{Expected Prediction Error}                      \\ \hline
Method                          & $\sigma_e^2$ (or $\sigma_u^2$) & Model                                      & Day 1 & Day 2 & Day 3 & Day 4 & Day 5 & $\sum_{h=1}^H{\rm OPE}(h)$ &  & Day 1 & Day 2 & Day 3 & Day 4 & Day 5 & $\sum_{h=1}^H{\rm EPE}(h)$ \\ \cline{1-9} \cline{11-16} 
                                &                                & \multicolumn{7}{l}{British Columbia}                                                                            &  &       &       &       &       &       &                            \\
Naive                           & -                              & \multicolumn{1}{c}{\multirow{5}{*}{\textbf{AR(1)}\tnote{a}}} & 0.015 & 0.015 & 0.032 & 0.043 & 0.020 & 0.126                      &  & 0.164 & 0.167 & 0.167 & 0.167 & 0.167 & 0.834                      \\
\multirow{2}{*}{Additive}       & Mild                           & \multicolumn{1}{c}{}                       & 0.010 & 0.005 & 0.011 & 0.011 & 0.000 & 0.037                      &  & 0.154 & 0.157 & 0.157 & 0.157 & 0.157 & 0.783                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.010 & 0.005 & 0.011 & 0.011 & 0.000 & 0.037                      &  & 0.154 & 0.157 & 0.157 & 0.157 & 0.157 & 0.784                      \\
\multirow{2}{*}{Multiplicative} & Mild                           & \multicolumn{1}{c}{}                       & 0.010 & 0.005 & 0.011 & 0.011 & 0.000 & 0.037                      &  & 0.044 & 0.044 & 0.044 & 0.044 & 0.044 & 0.222                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.010 & 0.005 & 0.011 & 0.011 & 0.000 & 0.037                      &  & 0.034 & 0.035 & 0.035 & 0.035 & 0.035 & 0.174                      \\ \cline{3-16} 
Naive                           & -                              & \multirow{5}{*}{AR(2)}                    & 0.016 & 0.014 & 0.031 & 0.042 & 0.019 & 0.122                      &  & 0.161 & 0.165 & 0.167 & 0.167 & 0.167 & 0.828                      \\
\multirow{2}{*}{Additive}       & Mild                           &                                            & 0.010 & 0.005 & 0.010 & 0.010 & 0.000 & 0.035                      &  & 0.151 & 0.155 & 0.157 & 0.157 & 0.157 & 0.777                      \\
                                & Moderate                       &                                            & 0.010 & 0.005 & 0.010 & 0.010 & 0.000 & 0.035                      &  & 0.151 & 0.155 & 0.157 & 0.157 & 0.157 & 0.778                      \\
\multirow{2}{*}{Multiplicative} & Mild                           &                                            & 0.010 & 0.005 & 0.010 & 0.010 & 0.000 & 0.035                      &  & 0.043 & 0.044 & 0.044 & 0.044 & 0.044 & 0.220                      \\
                                & Moderate                       &                                            & 0.010 & 0.005 & 0.010 & 0.010 & 0.000 & 0.034                      &  & 0.034 & 0.035 & 0.035 & 0.035 & 0.035 & 0.173                      \\ \hline
                                &                                & \multicolumn{7}{l}{Ontario}                                                                                     &  &       &       &       &       &       &                            \\
Naive                           & -                              & \multirow{5}{*}{\textbf{AR(1)}\tnote{a}}                    & 0.020 & 0.087 & 0.196 & 0.521 & 1.059 & 1.884                      &  & 2.527 & 2.643 & 2.649 & 2.649 & 2.649 & 13.117                     \\
\multirow{2}{*}{Additive}       & Mild                           &                                            & 0.001 & 0.004 & 0.007 & 0.056 & 0.175 & 0.243                      &  & 2.264 & 2.391 & 2.399 & 2.399 & 2.399 & 11.853                     \\
                                & Moderate                       &                                            & 0.000 & 0.000 & 0.000 & 0.023 & 0.110 & 0.134                      &  & 1.453 & 1.626 & 1.646 & 1.649 & 1.649 & 8.023                      \\
\multirow{2}{*}{Multiplicative} & Mild                           &                                            & 0.000 & 0.002 & 0.003 & 0.044 & 0.152 & 0.201                      &  & 0.558 & 0.599 & 0.603 & 0.603 & 0.603 & 2.965                      \\
                                & Moderate                       &                                            & 0.004 & 0.010 & 0.014 & 0.000 & 0.035 & 0.063                      &  & 0.270 & 0.331 & 0.345 & 0.348 & 0.348 & 1.642                      \\ \cline{3-16} 
Naive                           & -                              & \multicolumn{1}{c}{\multirow{5}{*}{AR(2)}} & 0.073 & 0.107 & 0.240 & 0.550 & 1.111 & 2.081                      &  & 2.517 & 2.648 & 2.648 & 2.649 & 2.649 & 13.111                     \\
\multirow{2}{*}{Additive}       & Mild                           & \multicolumn{1}{c}{}                       & 0.029 & 0.014 & 0.026 & 0.083 & 0.227 & 0.379                      &  & 2.256 & 2.398 & 2.398 & 2.399 & 2.399 & 11.851                     \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.045 & 0.008 & 0.031 & 0.063 & 0.221 & 0.368                      &  & 1.470 & 1.658 & 1.646 & 1.649 & 1.649 & 8.072                      \\
\multirow{2}{*}{Multiplicative} & Mild                           & \multicolumn{1}{c}{}                       & 0.034 & 0.012 & 0.027 & 0.076 & 0.222 & 0.370                      &  & 0.571 & 0.606 & 0.603 & 0.603 & 0.603 & 2.986                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.085 & 0.001 & 0.071 & 0.024 & 0.310 & 0.491                      &  & 0.454 & 0.469 & 0.415 & 0.390 & 0.375 & 2.103                      \\ \hline
                                &                                & \multicolumn{7}{l}{Quebec}                                                                                       &  &       &       &       &       &       &                            \\
Naive                           & -                              & \multicolumn{1}{c}{\multirow{5}{*}{\textbf{AR(1)}\tnote{a}}} & 0.163 & 0.607 & 1.357 & 2.289 & 3.294 & 7.709                      &  & 1.811 & 1.811 & 1.811 & 1.811 & 1.811 & 9.057                      \\
\multirow{2}{*}{Additive}       & Mild                           & \multicolumn{1}{c}{}                        & 0.061 & 0.216 & 0.479 & 0.778 & 1.053 & 2.587                      &  & 1.561 & 1.561 & 1.561 & 1.561 & 1.561 & 7.807                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                        & 0.060 & 0.215 & 0.478 & 0.776 & 1.051 & 2.580                      &  & 0.811 & 0.811 & 0.811 & 0.811 & 0.811 & 4.057                      \\
\multirow{2}{*}{Multiplicative} & Mild                           & \multicolumn{1}{c}{}                        & 0.061 & 0.216 & 0.479 & 0.778 & 1.053 & 2.586                      &  & 0.399 & 0.399 & 0.399 & 0.399 & 0.399 & 1.995                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                        & 0.060 & 0.215 & 0.477 & 0.776 & 1.050 & 2.578                      &  & 0.205 & 0.205 & 0.205 & 0.205 & 0.205 & 1.025                      \\ \cline{3-16} 
Naive                           & -                              & \multirow{5}{*}{AR(2)}                      & 0.129 & 0.524 & 1.226 & 2.115 & 3.085 & 7.079                      &  & 1.746 & 1.746 & 1.809 & 1.809 & 1.811 & 8.921                      \\
\multirow{2}{*}{Additive}       & Mild                           &                                             & 0.052 & 0.195 & 0.446 & 0.734 & 1.002 & 2.429                      &  & 1.375 & 1.375 & 1.447 & 1.447 & 1.451 & 7.096                      \\
                                & Moderate                       &                                             & 0.032 & 0.109 & 0.247 & 0.396 & 0.519 & 1.303                      &  & 0.413 & 0.413 & 0.407 & 0.407 & 0.402 & 2.043                      \\
\multirow{2}{*}{Multiplicative} & Mild                           &                                             & 0.051 & 0.190 & 0.438 & 0.723 & 0.988 & 2.390                      &  & 0.345 & 0.345 & 0.356 & 0.356 & 0.357 & 1.760                      \\
                                & Moderate                       &                                             & 0.038 & 0.141 & 0.333 & 0.560 & 0.774 & 1.847                      &  & 0.332 & 0.332 & 0.234 & 0.234 & 0.187 & 1.319                      \\ \hline
                                &                                & \multicolumn{7}{l}{Alberta}                                                                                      &  &       &       &       &       &       &                            \\
Naive                           & -                              & \multirow{5}{*}{ \textbf{AR(1)}\tnote{a}}                     & 0.002 & 0.007 & 0.027 & 0.055 & 0.070 & 0.160                      &  & 0.125 & 0.125 & 0.125 & 0.125 & 0.125 & 0.627                      \\
\multirow{2}{*}{Additive}       & Mild                           &                                             & 0.004 & 0.012 & 0.044 & 0.087 & 0.115 & 0.262                      &  & 0.115 & 0.115 & 0.115 & 0.115 & 0.115 & 0.577                      \\
                                & Moderate                       &                                             & 0.006 & 0.017 & 0.052 & 0.098 & 0.129 & 0.302                      &  & 0.035 & 0.035 & 0.035 & 0.035 & 0.035 & 0.177                      \\
\multirow{2}{*}{Multiplicative} & Mild                           &                                             & 0.004 & 0.012 & 0.044 & 0.087 & 0.115 & 0.263                      &  & 0.031 & 0.031 & 0.031 & 0.031 & 0.031 & 0.157                      \\
                                & Moderate                       &                                             & 0.005 & 0.013 & 0.045 & 0.089 & 0.118 & 0.270                      &  & 0.022 & 0.022 & 0.022 & 0.022 & 0.022 & 0.109                      \\ \cline{3-16} 
Naive                           & -                              & \multicolumn{1}{c}{\multirow{5}{*}{AR(2)}}  & 0.003 & 0.010 & 0.033 & 0.064 & 0.081 & 0.191                      &  & 0.122 & 0.122 & 0.125 & 0.125 & 0.125 & 0.621                      \\
\multirow{2}{*}{Additive}       & Mild                           & \multicolumn{1}{c}{}                        & 0.005 & 0.016 & 0.051 & 0.097 & 0.127 & 0.296                      &  & 0.112 & 0.112 & 0.115 & 0.115 & 0.115 & 0.570                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                        & 0.006 & 0.018 & 0.056 & 0.104 & 0.136 & 0.320                      &  & 0.081 & 0.081 & 0.085 & 0.085 & 0.085 & 0.419                      \\
\multirow{2}{*}{Multiplicative} & Mild                           & \multicolumn{1}{c}{}                        & 0.005 & 0.016 & 0.052 & 0.099 & 0.129 & 0.301                      &  & 0.030 & 0.031 & 0.031 & 0.031 & 0.031 & 0.155                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                        & 0.006 & 0.019 & 0.059 & 0.109 & 0.141 & 0.334                      &  & 0.022 & 0.022 & 0.022 & 0.022 & 0.022 & 0.109                      \\ \hline
\end{tabular}
\begin{tablenotes}
\item[a]{\scriptsize The selected model}
\end{tablenotes}


\end{threeparttable}
\end{sidewaystable}


==> tables/Tab_par_Def2.tex <==
\begin{sidewaystable}
\setlength\extrarowheight{1pt} % provide a bit more vertical whitespace
\centering
\captionsetup{size=small}
\scriptsize

\begin{threeparttable}
\caption[]{Definition 2: The parameter estimation under different measurement error models: the AR(2) model with ``no differencing" is used to fit the data of Ontario, the AR(1) model with ``order-1 differencing" is used to fit the data of Alberta, and the AR(2) model with ``order-1 differencing" is used to fit the data of British Columbia and Quebec.  }
\label{tab:par-Def-2}

\begin{tabular}{cccccccccccccccccc}
\hline
\multicolumn{1}{l}{}      & \multicolumn{1}{l}{}    &           & \multicolumn{3}{c}{British Columbia} &  & \multicolumn{3}{c}{Ontario} &  & \multicolumn{3}{c}{Quebec} &  & \multicolumn{3}{c}{Alberta} \\ \cline{1-6} \cline{8-10} \cline{12-14} \cline{16-18} 
Method                    & Error Degree            & Parameter & EST        & SE        & p-value     &  & EST     & SE     & p-value  &  & EST     & SE     & p-value &  & EST     & SE     & p-value  \\ \hline
\multirow{3}{*}{Naive}    & \multirow{3}{*}{-}      & $\phi_0$  & 0.062      & 0.034     & 0.097       &  & 2.126   & 1.388  & 0.138    &  & 0.225   & 0.058  & 0.001   &  & -0.013  & 0.022  & 0.561    \\
                          &                         & $\phi_1$  & -0.415     & 0.186     & 0.046       &  & 1.167   & 0.209  & $<$0.001 &  & -0.122  & 0.136  & 0.380   &  & -0.124  & 0.172  & 0.477    \\
                          &                         & $\phi_2$  & -0.254     & 0.185     & 0.195       &  & -0.370  & 0.140  & 0.014    &  & -0.309  & 0.092  & 0.003   &  & -       & -      & -        \\ \hline
                          &                         & $\phi_0$  & 0.034      & 0.020     & 0.114       &  & 1.146   & 0.759  & 0.144    &  & 0.174   & 0.042  & 0.000   &  & -0.007  & 0.012  & 0.567    \\
                          & Small ($\sigma_{e1}^2$) & $\phi_1$  & -0.432     & 0.201     & 0.053       &  & 1.173   & 0.216  & $<$0.001 &  & 0.124   & 0.032  & 0.001   &  & -0.131  & 0.185  & 0.486    \\
The Proposed Method       &                         & $\phi_2$  & -0.268     & 0.205     & 0.215       &  & -0.375  & 0.141  & 0.014    &  & -0.130  & 0.165  & 0.435   &  & -       & -      & -        \\ \cline{2-18} 
with Additive Error       &                         & $\phi_0$  & 0.036      & 0.024     & 0.164       &  & 1.138   & 0.747  & 0.140    &  & -0.327  & 0.096  & 0.002   &  & -0.007  & 0.012  & 0.554    \\
                          & Large ($\sigma_{e2}^2$) & $\phi_1$  & -0.497     & 0.265     & 0.085       &  & 1.189   & 0.239  & $<$0.001 &  & 0.162   & 0.044  & 0.001   &  & -0.158  & 0.247  & 0.529    \\
                          &                         & $\phi_2$  & -0.320     & 0.354     & 0.384       &  & -0.390  & 0.172  & 0.032    &  & 0.132   & 0.041  & 0.004   &  & -       & -      & -        \\ \hline
                          &                         & $\phi_0$  & 0.034      & 0.020     & 0.115       &  & 1.139   & 0.748  & 0.141    &  & -0.164  & 0.229  & 0.480   &  & -0.007  & 0.012  & 0.564    \\
                          & Small ($\sigma_{u1}^2$) & $\phi_1$  & -0.439     & 0.205     & 0.053       &  & 1.188   & 0.231  & $<$0.001 &  & -0.394  & 0.199  & 0.059   &  & -0.144  & 0.205  & 0.487    \\
The Proposed Method       &                         & $\phi_2$  & -0.273     & 0.204     & 0.205       &  & -0.389  & 0.162  & 0.024    &  & 0.128   & 0.042  & 0.006   &  & -       & -      & -        \\ \cline{2-18} 
with Multiplicative Error &                         & $\phi_0$  & 0.039      & 0.032     & 0.236       &  & 1.112   & 0.747  & 0.149    &  & 0.127   & 0.036  & 0.002   &  & -0.008  & 0.012  & 0.546    \\
                          & Large ($\sigma_{u2}^2$) & $\phi_1$  & -0.584     & 0.339     & 0.111       &  & 1.255   & 0.503  & 0.020    &  & -0.143  & 0.194  & 0.467   &  & -0.205  & 0.317  & 0.524    \\
                          &                         & $\phi_2$  & -0.393     & 0.322     & 0.245       &  & -0.451  & 0.510  & 0.384    &  & -0.353  & 0.111  & 0.004   &  & -       & -      & -        \\ \hline
\end{tabular}
\begin{tablenotes}
\end{tablenotes}


\end{threeparttable}
\end{sidewaystable}



==> tables/Tab_par_Def3.tex <==
\begin{table}[htbp]
\centering
\tiny
\caption{Definition 3:  The parameter estimation under different measurement error models: the AR(1) model with ``order-1 differencing" is used to fit the data of British Columbia and the AR(4) model with ``order-1 differencing" is used to fit the data of Ontario.}\label{tab:par-Def-3}
\begin{tabular}{cccccccccc}
\hline
                          &                                          &           & \multicolumn{3}{c}{British Columbia} &  & \multicolumn{3}{c}{Ontario} \\ \cline{1-6} \cline{8-10} 
Method                    & Error Degree                             & Parameter & EST        & SE        & p-value     &  & EST     & SE     & p-value  \\ \hline
\multirow{5}{*}{Naive}    & \multirow{5}{*}{-}                       & $\phi_0$  & 0.105      & 0.038     & 0.018       &  & 0.379   & 0.057  & $<$0.001 \\
                          &                                          & $\phi_1$  & -0.207     & 0.077     & 0.020       &  & -0.086  & 0.099  & 0.391    \\
                          &                                          & $\phi_2$  & -          & -         & -           &  & -0.287  & 0.106  & 0.012    \\
                          &                                          & $\phi_3$  & -          & -         & -           &  & -0.301  & 0.094  & 0.004    \\
                          &                                          & $\phi_4$  & -          & -         & -           &  & -0.284  & 0.078  & 0.001    \\ \hline
                          & \multirow{5}{*}{Small ($\sigma_{e1}^2$)} & $\phi_0$  & 0.057      & 0.021     & 0.021       &  & 0.206   & 0.031  & $<$0.001 \\
                          &                                          & $\phi_1$  & -0.213     & 0.086     & 0.029       &  & -0.088  & 0.100  & 0.383    \\
                          &                                          & $\phi_2$  & -          & -         & -           &  & -0.290  & 0.109  & 0.014    \\
                          &                                          & $\phi_3$  & -          & -         & -           &  & -0.303  & 0.094  & 0.003    \\
The Proposed Method       &                                          & $\phi_4$  & -          & -         & -           &  & -0.287  & 0.081  & 0.002    \\ \cline{2-10} 
with Additive Error       & \multirow{5}{*}{Large ($\sigma_{e2}^2$)} & $\phi_0$  & 0.058      & 0.021     & 0.017       &  & 0.212   & 0.036  & $<$0.001 \\
                          &                                          & $\phi_1$  & -0.234     & 0.147     & 0.137       &  & -0.102  & 0.123  & 0.417    \\
                          &                                          & $\phi_2$  & -          & -         & -           &  & -0.306  & 0.139  & 0.037    \\
                          &                                          & $\phi_3$  & -          & -         & -           &  & -0.318  & 0.107  & 0.006    \\
                          &                                          & $\phi_4$  & -          & -         & -           &  & -0.308  & 0.093  & 0.003    \\ \hline
                          & \multirow{5}{*}{Small ($\sigma_{u1}^2$)} & $\phi_0$  & 0.058      & 0.023     & 0.027       &  & 0.210   & 0.033  & $<$0.001 \\
                          &                                          & $\phi_1$  & -0.244     & 0.090     & 0.019       &  & -0.097  & 0.107  & 0.375    \\
                          &                                          & $\phi_2$  & -          & -         & -           &  & -0.300  & 0.117  & 0.016    \\
                          &                                          & $\phi_3$  & -          & -         & -           &  & -0.312  & 0.098  & 0.004    \\
The Proposed Method       &                                          & $\phi_4$  & -          & -         & -           &  & -0.300  & 0.087  & 0.002    \\ \cline{2-10} 
with Multiplicative Error & \multirow{5}{*}{Large ($\sigma_{u2}^2$)} & $\phi_0$  & 0.066      & 0.035     & 0.087       &  & 0.230   & 0.058  & 0.001    \\
                          &                                          & $\phi_1$  & -0.401     & 0.219     & 0.092       &  & -0.139  & 0.183  & 0.454    \\
                          &                                          & $\phi_2$  & -          & -         & -           &  & -0.347  & 0.213  & 0.116    \\
                          &                                          & $\phi_3$  & -          & -         & -           &  & -0.354  & 0.159  & 0.035    \\
                          &                                          & $\phi_4$  & -          & -         & -           &  & -0.361  & 0.149  & 0.023    \\ \hline
\end{tabular}
\end{table}

==> tables/Tab_par_sigmas.tex <==
\begin{sidewaystable}
\setlength\extrarowheight{1pt} % provide a bit more vertical whitespace
\centering
\captionsetup{size=small}
\small

\begin{threeparttable}
\caption[]{The parameter values of $\sigma_e^2$ or $\sigma_u^2$ for the measurement error model (\ref{eqn:measmodelClassic}) or (\ref{eqn:measmodelmultiplicative}) that are used for sensitivity analyses. }
\label{tab:par-sigmas}

\begin{tabular}{cccccccccccccc}
\hline
Definition                    & Error Model                   &  & \multicolumn{2}{c}{British Columbia} &  & \multicolumn{2}{c}{Ontario} &  & \multicolumn{2}{c}{Quebec} &  & \multicolumn{2}{c}{Alberta} \\ \hline
\multirow{6}{*}{Definition 1} &                               &  & \multicolumn{2}{c}{AR(1)}            &  & \multicolumn{2}{c}{AR(1)}   &  & \multicolumn{2}{c}{AR(1)}  &  & \multicolumn{2}{c}{AR(1)}   \\
                              & Additive ($\sigma_e^2$)       &  & 0.1             & 0.2                &  & 0.5         & 1             &  & 0.5        & 1             &  & 0.1        & 0.3            \\
                              & Multiplicative ($\sigma_u^2$) &  & 0.3             & 0.6                &  & 0.5         & 1             &  & 0.5        & 1             &  & 0.4        & 0.8            \\
                              &                               &  & \multicolumn{2}{c}{AR(2)\tnote{*}}           &  & \multicolumn{2}{c}{-}       &  & \multicolumn{2}{c}{-}      &  & \multicolumn{2}{c}{-}       \\
                              & Additive ($\sigma_e^2$)       &  & 0.1             & 0.2                &  & -           & -             &  & -          & -             &  & -          & -              \\
                              & Multiplicative ($\sigma_u^2$) &  & 0.01            & 0.02               &  & -           & -             &  & -          & -             &  & -          & -              \\
 \hline
\multirow{3}{*}{Definition 2} &                               &  & \multicolumn{2}{c}{AR(2)}            &  & \multicolumn{2}{c}{AR(2)\tnote{*}}  &  & \multicolumn{2}{c}{AR(2)}  &  & \multicolumn{2}{c}{AR(1)}   \\
                              & Additive ($\sigma_e^2$)       &  & 0.05            & 0.1                &  & 0.05        & 0.1           &  & 0.1        & 0.2           &  & 0.05       & 0.1            \\
                              & Multiplicative ($\sigma_u^2$) &  & 0.2             & 0.5                &  & 0.005       & 0.01          &  & 0.3        & 0.6           &  & 0.4        & 0.8            \\ \hline
\multirow{3}{*}{Definition 3} &                               &  & \multicolumn{2}{c}{AR(2)}            &  & \multicolumn{2}{c}{AR(4)}   &  & \multicolumn{2}{c}{-}      &  & \multicolumn{2}{c}{-}       \\
                              & Additive ($\sigma_e^2$)       &  & 0.03            & 0.06               &  & 0.02        & 0.05           &  & -          & -             &  & -          & -              \\
                              & Multiplicative ($\sigma_u^2$) &  & 0.3             & 0.6                &  & 0.1         & 0.2           &  & -          & -             &  & -          & -              \\ \hline
\end{tabular}
\begin{tablenotes}
\item[*]{\scriptsize The time series with no differencing}
\end{tablenotes}


\end{threeparttable}
\end{sidewaystable}


==> tables/Table_Canada.tex <==
\begin{table}[htbp]
\centering
\tiny
\caption{The parameter estimation of the autoregressive regression model under different degree of measurement error}\label{tab:TableCanada}
\begin{tabular}{cccccccccc}
\hline
\multicolumn{1}{l}{}            & \multicolumn{1}{l}{}         &           & \multicolumn{3}{c}{British Columbia} &  & \multicolumn{3}{c}{Ontario} \\ \cline{1-6} \cline{8-10} 
Model                           & Degree                       & Parameter & EST        & s.d.      & p-value     &  & EST     & s.d.   & p-value  \\ \hline
\multirow{3}{*}{Naive}          & \multirow{3}{*}{-}           & $\phi_0$  & 0.406      & 0.148     & 0.018       &  & 0.970   & 0.128  & 0.000    \\
                                &                              & $\phi_1$  & -0.226     & 0.159     & 0.180       &  & 0.025   & 0.100  & 0.804    \\
                                &                              & $\phi_2$  & 0.376      & 0.131     & 0.014       &  & 0.263   & 0.049  & <0.001    \\ \hline
\multirow{6}{*}{Additive}       & \multirow{3}{*}{Mild}        & $\phi_0$  & 0.217      & 0.084     & 0.024       &  & 0.521   & 0.111  & 0.000    \\
                                &                              & $\phi_1$  & -0.231     & 0.167     & 0.192       &  & 0.030   & 0.185  & 0.874    \\
                                &                              & $\phi_2$  & 0.390      & 0.152     & 0.024       &  & 0.223   & 0.050  & <0.001    \\ \cline{2-10} 
                                & \multirow{3}{*}{Substantial} & $\phi_0$  & 0.163      & 0.280     & 0.572       &  & 0.503   & 0.413  & 0.235    \\
                                &                              & $\phi_1$  & -0.233     & 0.627     & 0.716       &  & 0.064   & 0.756  & 0.933    \\
                                &                              & $\phi_2$  & 0.600      & 0.490     & 0.244       &  & 0.103   & 0.051  & 0.052    \\ \hline
\multirow{6}{*}{Multiplicative} & \multirow{3}{*}{Mild}        & $\phi_0$  & 0.217      & 0.084     & 0.025       &  & 0.522   & 0.098  & 0.000    \\
                                &                              & $\phi_1$  & -0.231     & 0.169     & 0.198       &  & 0.029   & 0.157  & 0.854    \\
                                &                              & $\phi_2$  & 0.391      & 0.148     & 0.021       &  & 0.066   & 0.014  & <0.001    \\ \cline{2-10} 
                                & \multirow{3}{*}{Substantial} & $\phi_0$  & 0.206      & 0.107     & 0.078       &  & 0.508   & 0.731  & 0.493    \\
                                &                              & $\phi_1$  & -0.242     & 0.210     & 0.272       &  & 0.054   & 1.377  & 0.969    \\
                                &                              & $\phi_2$  & 0.443      & 0.197     & 0.044       &  & 0.036   & 0.016  & 0.032    \\ \hline
\end{tabular}
\end{table}

==> tables/Table_Peh.tex <==
\begin{sidewaystable}
\setlength\extrarowheight{1pt} % provide a bit more vertical whitespace
\centering
\captionsetup{size=small}
\tiny

\begin{threeparttable}
\caption[]{The observed prediction error and expected prediction error for different lag order of autoregressive models.}
\label{Tab:TablePeh}

\begin{tabular}{lllccccccccccccc}
\hline
                                &                                &                                            & \multicolumn{6}{c}{Observed Prediction Error}                                          &  & \multicolumn{6}{c}{Expected Prediction Error}                      \\ \hline
Method                          & $\sigma_e^2$ (or $\sigma_u^2$) & Model                                      & Day 1                     & Day 2 & Day 3 & Day 4 & Day 5 & $\sum_{h=1}^H{\rm OPE}(h)$ &  & Day 1 & Day 2 & Day 3 & Day 4 & Day 5 & $\sum_{h=1}^H{\rm EPE}(h)$ \\ \cline{1-9} \cline{11-16} 
                                &                                & \multicolumn{7}{l}{British Columbia}                                                                                                &  &       &       &       &       &       &                            \\
Naive                           & -                              & \multicolumn{1}{c}{\multirow{5}{*}{AR(1)}} & \multicolumn{1}{l}{0.053} & 0.037 & 0.105 & 0.148 & 0.079 & 0.421                      &  & 0.207 & 0.234 & 0.237 & 0.238 & 0.238 & 1.153                      \\
\multirow{2}{*}{Additive}       & Mild                           & \multicolumn{1}{c}{}                       & 0.005                     & 0.000 & 0.009 & 0.029 & 0.004 & 0.046                      &  & 0.196 & 0.223 & 0.227 & 0.228 & 0.228 & 1.101                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.004                     & 0.000 & 0.009 & 0.028 & 0.004 & 0.045                      &  & 0.106 & 0.134 & 0.143 & 0.146 & 0.147 & 0.676                      \\
\multirow{2}{*}{Multiplicative} & Mild                           & \multicolumn{1}{c}{}                       & 0.005                     & 0.000 & 0.009 & 0.029 & 0.004 & 0.046                      &  & 0.057 & 0.065 & 0.066 & 0.066 & 0.066 & 0.321                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.005                     & 0.000 & 0.009 & 0.028 & 0.004 & 0.046                      &  & 0.049 & 0.056 & 0.058 & 0.058 & 0.058 & 0.278                      \\ \cline{3-16} 
Naive                           & -                              & \multirow{5}{*}{\textbf{AR(2)}\tnote{a}}            & 0.025                     & 0.082 & 0.110 & 0.146 & 0.074 & 0.437                      &  & 0.177 & 0.186 & 0.219 & 0.225 & 0.232 & 1.039                      \\
\multirow{2}{*}{Additive}       & Mild                           &                                            & 0.001                     & 0.001 & 0.008 & 0.027 & 0.003 & 0.040                      &  & 0.166 & 0.175 & 0.207 & 0.213 & 0.221 & 0.981                      \\
                                & Moderate                       &                                            & 0.001                     & 0.001 & 0.010 & 0.028 & 0.003 & 0.044                      &  & 0.064 & 0.067 & 0.093 & 0.098 & 0.111 & 0.433                      \\
\multirow{2}{*}{Multiplicative} & Mild                           &                                            & 0.001                     & 0.001 & 0.008 & 0.027 & 0.003 & 0.040                      &  & 0.049 & 0.051 & 0.060 & 0.062 & 0.064 & 0.287                      \\
                                & Moderate                       &                                            & 0.001                     & 0.001 & 0.009 & 0.026 & 0.003 & 0.040                      &  & 0.039 & 0.041 & 0.050 & 0.052 & 0.054 & 0.235                      \\ \cline{3-16} 
Naive                           & -                              & \multirow{5}{*}{AR(3)}                     & 0.000                     & 0.054 & 0.103 & 0.198 & 0.086 & 0.442                      &  & 0.168 & 0.184 & 0.185 & 0.186 & 0.187 & 0.910                      \\
\multirow{2}{*}{Additive}       & Mild                           &                                            & 0.028                     & 0.003 & 0.005 & 0.047 & 0.002 & 0.086                      &  & 0.156 & 0.172 & 0.172 & 0.173 & 0.175 & 0.848                      \\
                                & Moderate                       &                                            & 0.055                     & 0.002 & 0.001 & 0.068 & 0.003 & 0.129                      &  & 0.064 & 0.089 & 0.128 & 0.203 & 0.301 & 0.784                      \\
\multirow{2}{*}{Multiplicative} & Mild                           &                                            & 0.028                     & 0.003 & 0.005 & 0.047 & 0.002 & 0.086                      &  & 0.046 & 0.051 & 0.051 & 0.051 & 0.051 & 0.249                      \\
                                & Moderate                       &                                            & 0.034                     & 0.003 & 0.004 & 0.053 & 0.002 & 0.097                      &  & 0.039 & 0.044 & 0.043 & 0.042 & 0.042 & 0.210                      \\ \hline
                                &                                & \multicolumn{7}{l}{Ontario}                                                                                                         &  &       &       &       &       &       &                            \\
Naive                           & -                              & \multirow{5}{*}{\textbf{AR(1)}\tnote{a}}            & 0.084                     & 0.097 & 0.177 & 0.070 & 0.039 & 0.467                      &  & 0.263 & 0.264 & 0.264 & 0.264 & 0.264 & 1.318                      \\
\multirow{2}{*}{Additive}       & Mild                           &                                            & 0.023                     & 0.021 & 0.001 & 0.037 & 0.068 & 0.151                      &  & 0.223 & 0.224 & 0.224 & 0.224 & 0.224 & 1.118                      \\
                                & Moderate                       &                                            & 0.014                     & 0.020 & 0.001 & 0.037 & 0.068 & 0.141                      &  & 0.103 & 0.104 & 0.104 & 0.104 & 0.104 & 0.518                      \\
\multirow{2}{*}{Multiplicative} & Mild                           &                                            & 0.023                     & 0.021 & 0.001 & 0.037 & 0.068 & 0.151                      &  & 0.066 & 0.066 & 0.066 & 0.066 & 0.066 & 0.331                      \\
                                & Moderate                       &                                            & 0.017                     & 0.021 & 0.001 & 0.037 & 0.068 & 0.144                      &  & 0.036 & 0.036 & 0.036 & 0.036 & 0.036 & 0.179                      \\ \cline{3-16} 
Naive                           & -                              & \multicolumn{1}{c}{\multirow{5}{*}{AR(2)}} & 0.038                     & 0.113 & 0.173 & 0.071 & 0.039 & 0.434                      &  & 0.259 & 0.259 & 0.263 & 0.263 & 0.264 & 1.308                      \\
\multirow{2}{*}{Additive}       & Mild                           & \multicolumn{1}{c}{}                       & 0.111                     & 0.008 & 0.003 & 0.036 & 0.068 & 0.226                      &  & 0.218 & 0.218 & 0.223 & 0.223 & 0.224 & 1.107                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.264                     & 0.002 & 0.017 & 0.021 & 0.081 & 0.386                      &  & 0.094 & 0.095 & 0.102 & 0.103 & 0.103 & 0.498                      \\
\multirow{2}{*}{Multiplicative} & Mild                           & \multicolumn{1}{c}{}                       & 0.109                     & 0.008 & 0.002 & 0.036 & 0.068 & 0.224                      &  & 0.065 & 0.065 & 0.066 & 0.066 & 0.066 & 0.329                      \\
                                & Moderate                       & \multicolumn{1}{c}{}                       & 0.212                     & 0.000 & 0.010 & 0.027 & 0.074 & 0.323                      &  & 0.036 & 0.036 & 0.036 & 0.036 & 0.036 & 0.180                      \\ \hline
\end{tabular}

\begin{tablenotes}
\item[a]{\scriptsize The selected model}
\end{tablenotes}


\end{threeparttable}
\end{sidewaystable}


==> tables/Table_alpha0.tex <==
\begin{table}[htbp]
\centering
\tiny
\caption{The parameter estimation of the autoregressive regression model with different $\alpha_0$}\label{tab:Tablealpha0}
\begin{tabular}{lccccccccc}
\hline
                          & \multicolumn{1}{l}{}  &           & \multicolumn{3}{c}{Time Series 1}                   &  & \multicolumn{3}{c}{Time Series 2}                    \\ \cline{1-6} \cline{8-10} 
Model                     & $\alpha_0$            & Parameter & Point Estimation (s.d.) & p-value & CI              &  & Point Estimation (s.d.) & p-value & CI               \\ \hline
\multirow{2}{*}{Naive}    & -                     & $\phi_0$  & 0.440 (0.112)           & 0.002   & (0.197, 0.683)  &  & -0.144 (0.049)          & 0.005   & (-0.242, -0.046) \\
                          & -                     & $\phi_1$  & -0.286 (0.157)          & 0.093   & (-0.629, 0.056) &  & -0.271 (0.053)          & 0.000   & (-0.378, -0.163) \\ \hline
\multirow{8}{*}{Additive} & \multirow{2}{*}{0}    & $\phi_0$  & 0.458 (0.120)           & 0.002   & (0.196, 0.719)  &  & -0.148 (0.051)          & 0.006   & (-0.252, -0.044) \\
                          &                       & $\phi_1$  & -0.338 (0.189)          & 0.098   & (-0.749, 0.073) &  & -0.303 (0.055)          & 0.000   & (-0.414, -0.192) \\ \cline{2-10} 
                          & \multirow{2}{*}{0.01} & $\phi_0$  & 0.444 (0.117)           & 0.002   & (0.190, 0.699)  &  & -0.161 (0.050)          & 0.003   & (-0.262, -0.060) \\
                          &                       & $\phi_1$  & -0.338 (0.186)          & 0.095   & (-0.744, 0.068) &  & -0.303 (0.053)          & 0.000   & (-0.410, -0.195) \\ \cline{2-10} 
                          & \multirow{2}{*}{0.05} & $\phi_0$  & 0.391 (0.111)           & 0.004   & (0.150, 0.632)  &  & -0.213 (0.049)          & 0.000   & (-0.312, -0.114) \\
                          &                       & $\phi_1$  & -0.338 (0.189)          & 0.099   & (-0.749, 0.073) &  & -0.303 (0.054)          & 0.000   & (-0.412, -0.194) \\ \cline{2-10} 
                          & \multirow{2}{*}{0.1}  & $\phi_0$  & 0.324 (0.104)           & 0.009   & (0.097, 0.551)  &  & -0.278 (0.048)          & 0.000   & (-0.375, -0.182) \\
                          &                       & $\phi_1$  & -0.338 (0.189)          & 0.099   & (-0.749, 0.073) &  & -0.303 (0.054)          & 0.000   & (-0.412, -0.194) \\ \hline
\end{tabular}
\end{table}

==> tables/Table_sigmas.tex <==
\begin{table}[htbp]
\centering
\tiny
\caption{The parameter estimation of the autoregressive regression model under different degree of measurement error}\label{tab:TableAR}
\begin{tabular}{llcccccccc}
\hline
                                &                              &           & \multicolumn{3}{c}{Time Series 1}             &  & \multicolumn{3}{c}{Time Series 2}              \\ \cline{4-6} \cline{8-10} 
Model                           & Degree                       & Parameter & Estimates (s.e.) & P-value  & CI              &  & Estimates (s.e.) & P-value  & CI               \\ \hline
\multirow{2}{*}{Naive}          & \multirow{2}{*}{-}           & $\phi_0$  & -0.144 (0.097)   & 0.163    & (-0.356, 0.067) &  & -0.144 (0.067)   & 0.036    & (-0.279, -0.010) \\
                                &                              & $\phi_1$  & -0.271 (0.155)   & 0.106    & (-0.608, 0.067) &  & -0.271 (0.064)   & $<$0.001 & (-0.399, -0.142) \\ \hline
\multirow{6}{*}{Additive}       & \multirow{2}{*}{Mild}        & $\phi_0$  & 0.422 (0.096)    & $<$0.001 & (0.212, 0.631)  &  & -0.145 (0.064)   & 0.030    & (-0.275, -0.015) \\
                                &                              & $\phi_1$  & -0.283 (0.154)   & 0.092    & (-0.620, 0.053) &  & -0.278 (0.068)   & $<$0.001 & (-0.416, -0.140) \\ \cline{3-10} 
                                & \multirow{2}{*}{Moderate}    & $\phi_0$  & 0.439 (0.103)    & $<$0.001 & (0.214, 0.664)  &  & -0.154 (0.069)   & 0.032    & (-0.294, -0.014) \\
                                &                              & $\phi_1$  & -0.335 (0.174)   & 0.078    & (-0.714, 0.044) &  & -0.355 (0.073)   & $<$0.001 & (-0.502, -0.209) \\ \cline{3-10} 
                                & \multirow{2}{*}{Substantial} & $\phi_0$  & 0.596 (0.350)    & 0.114    & (-0.166, 1.357) &  & -0.180 (0.159)   & 0.266    & (-0.502, 0.142)  \\
                                &                              & $\phi_1$  & -0.812 (1.070)   & 0.462    & (-3.145, 1.520) &  & -0.585 (0.954)   & 0.543    & (-2.512, 1.342)  \\ \hline
\multirow{6}{*}{Multiplicative} & \multirow{2}{*}{Mild}        & $\phi_0$  & 0.422 (0.098)    & $<$0.001 & (0.209, 0.636)  &  & -0.146 (0.066)   & 0.032    & (-0.278, -0.013) \\
                                &                              & $\phi_1$  & -0.284 (0.157)   & 0.096    & (-0.627, 0.058) &  & -0.282 (0.067)   & $<$0.001 & (-0.418, -0.146) \\ \cline{3-10} 
                                & \multirow{2}{*}{Moderate}    & $\phi_0$  & 0.458 (0.123)    & $<$0.001 & (0.189, 0.727)  &  & -0.160 (0.073)   & 0.034    & (-0.308, -0.012) \\
                                &                              & $\phi_1$  & -0.394 (0.225)   & 0.106    & (-0.884, 0.097) &  & -0.410 (0.095)   & $<$0.001 & (-0.602, -0.218) \\ \cline{3-10} 
                                & \multirow{2}{*}{Substantial} & $\phi_0$  & 0.635 (0.327)    & 0.076    & (-0.078, 1.348) &  & -0.184 (0.086)   & 0.039    & (-0.359, -0.010) \\
                                &                              & $\phi_1$  & -0.932 (0.716)   & 0.218    & (-2.493, 0.629) &  & -0.624 (0.138)   & $<$0.001 & (-0.902, -0.345) \\ \hline
\end{tabular}
\end{table}
